Sports-Traj: A Unified Trajectory Generation Model for Multi-Agent Movement in Sports

Understanding multi-agent movement is critical across various fields. The conventional approaches typically focus on separate tasks such as trajectory prediction, imputation, or spatial-temporal recovery. Considering the unique formulation and constraint of each task, most existing methods are tailored for only one, limiting the ability to handle multiple tasks simultaneously, which is a common requirement in real-world scenarios. Another limitation is that widely used public datasets mainly focus on pedestrian movements with casual, loosely connected patterns, where interactions between individuals are not always present, especially at a long distance, making them less representative of more structured environments. To overcome these limitations, we propose a Unified Trajectory Generation model, UniTraj, that processes arbitrary trajectories as masked inputs, adaptable to diverse scenarios in the domain of sports games. Specifically, we introduce a Ghost Spatial Masking (GSM) module, embedded within a Transformer encoder, for spatial feature extraction. We further extend recent State Space Models (SSMs), known as the Mamba model, into a Bidirectional Temporal Mamba (BTM) to better capture temporal dependencies. Additionally, we incorporate a Bidirectional Temporal Scaled (BTS) module to thoroughly scan trajectories while preserving temporal missing relationships. Furthermore, we curate and benchmark three practical sports datasets, Basketball-U, Football-U, and Soccer-U, for evaluation. Extensive experiments demonstrate the superior performance of our model. We hope that our work can advance the understanding of human movement in real-world applications, particularly in sports. Our datasets, code, and model weights are available here https://github.com/colorfulfuture/UniTraj-pytorch.

==> contents/4_preliminary.tex <==

\section{Preliminary}
{\color{blue}
\paragraph{Selective Structured State Space Sequence Model.}
SSMs particularly through the contributions of structured state space sequence models (S4) and Mamba, have demonstrated exceptional proficiency in handling long sequences. These models operationalize the mapping of a 1-D function or sequence, $x(t) \in \mathbb{R} \mapsto y(t) \in \mathbb{R}$, through a hidden state $h(t) \in \mathbb{R}^N$, employing $\mathbf{A} \in \mathbb{R}^{N \times N}$ as the evolution parameters, $\mathbf{B} \in \mathbb{R}^{N \times 1}$ and $\mathbf{C} \in \mathbb{R}^{1 \times N}$ as the projection parameters, respectively.
The continuous system dynamics are described by the ordinary differential equation (ODE):
\begin{equation}
\begin{aligned}
h'(t) &= \mathbf{A}h(t) + \mathbf{B}x(t), \\
y(t) &= \mathbf{C}h(t) + \mathbf{D}x(t),
\end{aligned}
\end{equation}
with $x(t)$ representing a continuous input signal and $y(t)$ a continuous output signal in the time domain.

To adapt these continuous dynamics for practical computation, the S4 and Mamba models employ a discretization process, notably using the zero-order hold (ZOH) method, resulting in a transformation of continuous parameters into discrete ones:
\begin{equation}
\begin{aligned}
\mathbf{\overline{A}} &= \exp{(\mathbf{\Delta}\mathbf{A})}, \\
\mathbf{\overline{B}} &= (\mathbf{\Delta} \mathbf{A})^{-1}(\exp{(\mathbf{\Delta} \mathbf{A})} - \mathbf{I}) \cdot \mathbf{\Delta} \mathbf{B}.
\end{aligned}
\end{equation}
The discretized system can then be expressed as follows, incorporating a step size $\mathbf{\Delta}$:
\begin{equation}
\begin{aligned}
h_t &= \mathbf{\overline{A}}h_{t-1} + \mathbf{\overline{B}}x_{t}, \\
y_t &= \mathbf{C}h_t.
\end{aligned}
\end{equation}
This adaptation facilitates the computation of output through global convolution, leveraging a structured convolutional kernel $\overline{\mathbf{K}}$, which encompasses the entire length $M$ of the input sequence $\mathbf{x}$:
\begin{equation}
\begin{aligned}
\mathbf{\overline{K}} &= (\mathbf{C}\mathbf{\overline{B}}, \mathbf{C}\mathbf{\overline{A}}\mathbf{\overline{B}}, \dots, \mathbf{C}\mathbf{\overline{A}}^{M-1}\mathbf{\overline{B}}), \\
\mathbf{y} &= \mathbf{x} * \mathbf{\overline{K}}.
\end{aligned}
\label{eq:ssm}
\end{equation}
Selective models like Mamba introduce time-varying parameters, deviating from the linear time invariance (LTI) assumption and complicating parallel computation. However, hardware-aware optimizations, such as associative scans, have been developed to address these computational challenges, highlighting the ongoing evolution and application of SSMs in modeling complex temporal dynamics.

}

==> tables/results_ablation_study_deprecated.tex <==
\begin{wraptable}{l}{0.6\textwidth}
\centering
  \caption{}
  \label{tab:results_ablation_study} 
  \scalebox{0.75}{
    \begin{tabular}{l|c|c|c}
    \toprule
    \multirow{2}{*}{Variants} & \multicolumn{3}{c}{minADE$_{20}$ $\downarrow$} \\ 
    \cmidrule(lr){2-4}
    
    & \textbf{\textit{Basketball-U}} & \textbf{\textit{Football-U}}&  \textbf{\textit{Soccer-U}} \\
    
    \midrule
     w/o GSM & 4.86 & 3.92 & 119.43\\
     w/o BTS & 4.86 & 3.60 & 105.47\\
     uni w/ GSM & 5.86 & 4.09 & 106.22\\
     uni w/o GSM & 5.86 & 4.10 & 113.49\\
    \cmidrule(lr){1-4}
    \rowcolor{RowColor} 
    \textbf{whole (ours)} 
    & \textbf{4.77} 
    & \textbf{3.55}
    & \textbf{94.59} \\
    \bottomrule
  \end{tabular}
  }
\end{wraptable}


==> tables/results_head_embedding_deprecated..tex <==
\begin{wraptable}{l}{0.48\textwidth}
\centering
  \caption{}
  \label{tab:results_head_embedding} 
  \scalebox{0.75}{
    \begin{tabular}{l|c|c|c}
    \toprule
    \multirow{2}{*}{Variants} & \multicolumn{3}{c}{minADE$_{20}$ $\downarrow$} \\ 
    \cmidrule(lr){2-4}
    
    & \textbf{\textit{Basketball-U}} & \textbf{\textit{Football-U}}&  \textbf{\textit{Soccer-U}} \\
    
    \midrule
    w/ global & 4.86 & 3.74 & 106.77\\
    w/ learnable & 4.92 & 3.63 & 107.50\\
    \cmidrule(lr){1-4}
    w/ mean & 4.80 & 3.64 & 100.84\\
    w/ sum & 4.79 & 3.56 & 102.99\\
    \rowcolor{RowColor} 
    \textbf{w/ max (ours)} 
    & \textbf{4.77} 
    & \textbf{3.55}
    & \textbf{94.59} \\
    \bottomrule
  \end{tabular}
  }
\end{wraptable}

